YouTube, The Great Radicalizer? Auditing and Mitigating Ideological Biases in YouTube Recommendations

Recommendations algorithms of social media platforms are often criticized for placing users in "rabbit holes" of (increasingly) ideologically biased content. Despite these concerns, prior evidence on this algorithmic radicalization is inconsistent. Furthermore, prior work lacks systematic interventions that reduce the potential ideological bias in recommendation algorithms. We conduct a systematic audit of YouTube's recommendation system using a hundred thousand sock puppets to determine the presence of ideological bias (i.e., are recommendations aligned with users' ideology), its magnitude (i.e., are users recommended an increasing number of videos aligned with their ideology), and radicalization (i.e., are the recommendations progressively more extreme). Furthermore, we design and evaluate a bottom-up intervention to minimize ideological bias in recommendations without relying on cooperation from YouTube. We find that YouTube's recommendations do direct users -- especially right-leaning users -- to ideologically biased and increasingly radical content on both homepages and in up-next recommendations. Our intervention effectively mitigates the observed bias, leading to more recommendations to ideologically neutral, diverse, and dissimilar content, yet debiasing is especially challenging for right-leaning users. Our systematic assessment shows that while YouTube recommendations lead to ideological bias, such bias can be mitigated through our intervention.

==> figures/rl_mdp_tikz.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,367); %set diagram left start at 0, and has height of 367

%Shape: Rectangle [id:dp07025444510338152] 
\draw  [line width=2.25]  (280,48) -- (366,48) -- (366,99) -- (280,99) -- cycle ;
%Shape: Rectangle [id:dp7806979063324857] 
\draw  [line width=2.25]  (280,205) -- (366,205) -- (366,256) -- (280,256) -- cycle ;
%Straight Lines [id:da04540884544148227] 
\draw    (367,76) -- (436,76) ;
%Straight Lines [id:da091515285401093] 
\draw    (436,76) -- (436,234) ;
%Straight Lines [id:da3583461145097473] 
\draw    (436,234) -- (369,234) ;
\draw [shift={(367,234)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9522448043637604] 
\draw    (276.6,219) -- (76,218.62) ;
%Straight Lines [id:da4750339987641905] 
\draw    (76,218.62) -- (78.77,89) ;
%Straight Lines [id:da6716315903137065] 
\draw    (78.77,89) -- (278,89) ;
\draw [shift={(280,89)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5543354872327659] 
\draw    (280,249) -- (48,248.45) ;
%Straight Lines [id:da15383947291944167] 
\draw    (48,248.45) -- (51.29,57) ;
%Straight Lines [id:da7271068173742015] 
\draw    (51.29,57) -- (275.77,57.99) ;
\draw [shift={(277.77,58)}, rotate = 180.25] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3586907648669524] 
\draw    (280,249) -- (101,248.01) ;
\draw [shift={(99,248)}, rotate = 360.32] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1261195378004154] 
\draw    (278.12,219) -- (101,218.01) ;
\draw [shift={(99,218)}, rotate = 360.32] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6698447858493914] 
\draw    (97.5,192) .. controls (99.17,193.67) and (99.17,195.33) .. (97.5,197) .. controls (95.83,198.67) and (95.83,200.33) .. (97.5,202) .. controls (99.17,203.67) and (99.17,205.33) .. (97.5,207) .. controls (95.83,208.67) and (95.83,210.33) .. (97.5,212) .. controls (99.17,213.67) and (99.17,215.33) .. (97.5,217) .. controls (95.83,218.67) and (95.83,220.33) .. (97.5,222) .. controls (99.17,223.67) and (99.17,225.33) .. (97.5,227) .. controls (95.83,228.67) and (95.83,230.33) .. (97.5,232) .. controls (99.17,233.67) and (99.17,235.33) .. (97.5,237) .. controls (95.83,238.67) and (95.83,240.33) .. (97.5,242) .. controls (99.17,243.67) and (99.17,245.33) .. (97.5,247) .. controls (95.83,248.67) and (95.83,250.33) .. (97.5,252) .. controls (99.17,253.67) and (99.17,255.33) .. (97.5,257) .. controls (95.83,258.67) and (95.83,260.33) .. (97.5,262) .. controls (99.17,263.67) and (99.17,265.33) .. (97.5,267) .. controls (95.83,268.67) and (95.83,270.33) .. (97.5,272) .. controls (99.17,273.67) and (99.17,275.33) .. (97.5,277) -- (97.5,277)(94.5,192) .. controls (96.17,193.67) and (96.17,195.33) .. (94.5,197) .. controls (92.83,198.67) and (92.83,200.33) .. (94.5,202) .. controls (96.17,203.67) and (96.17,205.33) .. (94.5,207) .. controls (92.83,208.67) and (92.83,210.33) .. (94.5,212) .. controls (96.17,213.67) and (96.17,215.33) .. (94.5,217) .. controls (92.83,218.67) and (92.83,220.33) .. (94.5,222) .. controls (96.17,223.67) and (96.17,225.33) .. (94.5,227) .. controls (92.83,228.67) and (92.83,230.33) .. (94.5,232) .. controls (96.17,233.67) and (96.17,235.33) .. (94.5,237) .. controls (92.83,238.67) and (92.83,240.33) .. (94.5,242) .. controls (96.17,243.67) and (96.17,245.33) .. (94.5,247) .. controls (92.83,248.67) and (92.83,250.33) .. (94.5,252) .. controls (96.17,253.67) and (96.17,255.33) .. (94.5,257) .. controls (92.83,258.67) and (92.83,260.33) .. (94.5,262) .. controls (96.17,263.67) and (96.17,265.33) .. (94.5,267) .. controls (92.83,268.67) and (92.83,270.33) .. (94.5,272) .. controls (96.17,273.67) and (96.17,275.33) .. (94.5,277) -- (94.5,277) ;

% Text Node
\draw (291,63) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{47.49pt}\setlength\topsep{0pt}
\begin{center}
\textbf{RL Agent}
\end{center}

\end{minipage}};
% Text Node
\draw (291,212) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{44.84pt}\setlength\topsep{0pt}
\begin{center}
\textbf{User's }\\\textbf{YouTube}
\end{center}

\end{minipage}};
% Text Node
\draw    (444,103) -- (506,103) -- (506,129) -- (444,129) -- cycle  ;
\draw (447,107.4) node [anchor=north west][inner sep=0.75pt]    {$a_{t} \ \in \ A$};
% Text Node
\draw (442,138) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{\textbf{Action: }}\\Watch/Inject Video};
% Text Node
\draw    (115,255) -- (241,255) -- (241,281) -- (115,281) -- cycle  ;
\draw (118,259.4) node [anchor=north west][inner sep=0.75pt]    {$s_{t}{}_{+}{}_{1} \ =\ \Delta ( H_{t}{}_{+}{}_{1})$};
% Text Node
\draw    (114,183) -- (258,183) -- (258,209) -- (114,209) -- cycle  ;
\draw (117,187.4) node [anchor=north west][inner sep=0.75pt]    {$r_{t}{}_{+}{}_{1} \ =\ -\mathcal{O}( H_{t}{}_{+}{}_{1})$};
% Text Node
\draw    (222,28) -- (242,28) -- (242,54) -- (222,54) -- cycle  ;
\draw (225,32.4) node [anchor=north west][inner sep=0.75pt]    {$s_{t}$};
% Text Node
\draw    (223,93) -- (243,93) -- (243,119) -- (223,119) -- cycle  ;
\draw (226,97.4) node [anchor=north west][inner sep=0.75pt]    {$r_{t}$};
% Text Node
\draw (124,158) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{\textbf{Reward Obtained}}};
% Text Node
\draw (115,292) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{\textit{Next State: }}Top-k Homepage Video Slant Scores};
% Text Node
\draw (98,32) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{\textit{Previous State}}};
% Text Node
\draw (88,96) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{\textit{Previous Reward}}};


\end{tikzpicture}


==> tables/table-pathways.tex <==
\begin{table*}[t]
  \caption{Percentage of consecutive video watches during testing for each sock-puppet that either radicalize, de-radicalize, or remain stagnant}
  \label{tab:radicalization-pathways}

\begin{tabular}{llllll}
\toprule
{} &    Left radicalize &   Right radicalize &  Left deradicalize & Right deradicalize &           Stagnant \\
\midrule
Far Left  &  $28.5\% \pm 26.2\%$ &  $14.0\% \pm 20.3\%$ &  $22.7\% \pm 24.5\%$ &  $11.7\% \pm 19.5\%$ &  $23.0\% \pm 26.3\%$ \\
Left      &  $25.5\% \pm 25.8\%$ &  $17.3\% \pm 23.0\%$ &  $20.5\% \pm 24.0\%$ &  $14.8\% \pm 22.4\%$ &  $21.8\% \pm 25.0\%$ \\
Moderate  &  $24.1\% \pm 26.5\%$ &  $18.8\% \pm 23.4\%$ &  $17.6\% \pm 23.7\%$ &  $15.3\% \pm 21.3\%$ &  $24.1\% \pm 26.7\%$ \\
Right     &  $22.6\% \pm 24.1\%$ &  $18.5\% \pm 21.4\%$ &  $17.4\% \pm 22.4\%$ &  $16.9\% \pm 21.7\%$ &  $24.6\% \pm 25.5\%$ \\
Far Right &  $18.0\% \pm 21.0\%$ &  $21.5\% \pm 21.3\%$ &  $13.6\% \pm 20.0\%$ &  $17.6\% \pm 19.9\%$ &  $29.4\% \pm 26.6\%$ \\
\bottomrule
\end{tabular}
\textbf{}


\end{table*}

==> tables/table-slant-intervals.tex <==
\begin{table}
  \caption{Interval range for slant estimates}
  \label{tab:slant-intervals}
  \begin{tabular}{lc}
    \toprule
    Category & Interval \\
    \midrule
    \lbin & $-1.0 \rightarrow -0.6$\\
    \clbin & $-0.6 \rightarrow -0.2$\\
    \cbin & $-0.2 \rightarrow +0.2$\\
    \crbin & $+0.2 \rightarrow +0.6$\\
    \rbin & $+0.6 \rightarrow +1.0$\\
    \bottomrule
  \end{tabular}
\end{table}

==> tables/table-slant-transitions.tex <==
\begin{table}
  \caption{Transition types between consecutively watched videos with slant $t_0$ and $t_1$}
  \label{tab:slant-transitions}
  \begin{tabular}{ll}
    \toprule
    Transition & Ruling \\
    \midrule
    Left-radicalizing & $t_1<t_0 \land t_1<-0.2 \land |t_1 - t_0| > 0.1$ \\
    Right-radicalizing & $t_1 > t_0 \land t_1 > 0.2 \land |t_1 - t_0| > 0.1$\\
    Left-deradicalizing & $t_1 > t_0 \land t_1 < -0.2 \land |t_1 - t_0| > 0.1$\\
    Right-deradicalizing & $t_1 < t_0 \land t_1 > 0.2 \land |t_1 - t_0| > 0.1$\\
    Stagnant & $|t_1 - t_0| < 0.1$ \\
    \bottomrule
  \end{tabular}
\end{table}


%  Left radicalization
% t_1 < t_0 and t_1 < -0.2
% Right radicalization

% Left deradicalization
% $t_1 > t_0 \land t_1 < -0.2$
% % Right deradicalization
% $t_1 < t_0 \land t_1 > 0.2$

